Designing an Automated Vehicle: Strategies for Handling Tasks of a Previously Required Accompanying Person

When using a conventional passenger car, several groups of people are reliant on the assistance of an accompanying person, for example when getting in and out of the car. For the independent use of an automatically driving vehicle by those groups, the absence of a previously required accompanying person needs to be compensated. During the design process of an autonomous family vehicle, we found that a low-barrier vehicle design can only partly contribute to the compensation for the absence of a required human companion. In this paper, we present four strategies we identified for handling the tasks of a previously required accompanying individual. The presented top-down approach supports developers in identifying unresolved problems, in finding, structuring, and selecting solutions as well as in uncovering upcoming problems at an early stage in the development of novel concepts for driverless vehicles. As an example, we consider the hypothetical exit of persons in need of assistance. The application of the four strategies in this example demonstrates the far-reaching impact of consistently considering users in need of support in the development of automated vehicles.

==> results.tex <==
\label{sec:results}


\subsection{Simulation set-up}
\label{subsec:simulation}
The evaluation is conducted in the CarMaker simulation environment which features complex multi-body vehicle models \cite{ipgautomotivegmbh_2019}. 
We adopted a standard vehicle to over-actuated capabilities with four individually controllable steering, drive, as well as brake actuators. 
Moreover, we added the capability to model a freely running wheel without any applied forces and moments stemming from steering, brake, and drive following \cite[pp. 35]{halfmann_2003}. 
\begin{figure}
	\centering
	\includegraphics[width=\linewidth]{figures/MOBILECarMaker}
	\caption{The experimental vehicle \textsc{Mobile} in the CarMaker simulation environment}
	\label{fig:CarMaker}
\end{figure}

The vehicle was parameterized similar to our experimental vehicle \textsc{Mobile}. 
The simulation parameters, the controller algorithm's weights and constraints are described in the appendix. 
Moreover, we assume a degradation detection and isolation time $\Delta t_\mathrm{DDI}=\SI{0.2}{\second}$ after degradation occurrence. 


%\pgfplotstableread[col sep=comma]{figures/reference2.csv}{\referencetrajectory}
%\pgfplotstablegetrowsof{\referencetrajectory}
%\pgfmathsetmacro\lastrow{\pgfplotsretval-1}
%\pgfplotstablegetcolsof{\referencetrajectory}
%\pgfmathsetmacro\lastcol{\pgfplotsretval-1}
%
%\begin{table*}
%	\pgfplotstabletypeset[]{\referencetrajectory}
%\end{table*}

\pgfplotstableread[col sep=comma]{figures/reference2.csv}{\referencetrajectory}
\pgfplotstablegetrowsof{\referencetrajectory}
\pgfmathsetmacro\lastrow{\pgfplotsretval-1}
\pgfplotstablegetcolsof{\referencetrajectory}
\pgfmathsetmacro\lastcol{\pgfplotsretval-1}

%\begin{table*}
%	\pgfplotstabletypeset[]{\referencetrajectory}
%\end{table*}

\begin{figure*}
	\centering
	\input{figures/trajectory.tikz}
	\label{fig:trajectory_normal}
	\caption{Trajectory without degradation}
\end{figure*}

\begin{table*}
	\centering
	\label{fig:trajectory_normal}%
	\caption{Trajectory without degradation}%
	\input{tables/results.tikz}
\end{table*}


\subsection{Trajectory tracking}
\label{subsec:normaloperation}


Normale Trajektorie, Ackermannlenkwinkel? 

Kurze Erwähnung, dass das Wissen über die Radaufstandskräfte wichtig ist (Vergleich mit und ohne Wissen (Messung/Modellbasiert))

Trajektorie mit Schwimmwinkel und ohne Gierrate

Robustheit gegen Parametervariation ($m$, $J$, $\mu$, Reifenparameter)

Robustheit gegen noisy inputs

Robustheit gegen Steigungen

\subsection{Degraded operation}
\label{subsec:degradaedoperation}
